Simple Strategies in Multi-Objective MDPs (Technical Report)

We consider the verification of multiple expected reward objectives at once on Markov decision processes (MDPs). This enables a trade-off analysis among multiple objectives by obtaining the Pareto front. We focus on strategies that are easy to employ and implement. That is, strategies that are pure (no randomization) and have bounded memory. We show that checking whether a point is achievable by a pure stationary strategy is NP-complete, even for two objectives, and we provide an MILP encoding to solve the corresponding problem. The bounded memory case can be reduced to the stationary one by a product construction. Experimental results using \Storm and Gurobi show the feasibility of our algorithms.

==> boundedmem.tex <==
%!TEX root = ./paper.tex
\section{Bounded Memory}
\label{sec:boundedmem}
%\tq{Add motivation that unbounded memory is intractable?}

As motivated in introduction, we want to construct simple schedulers that are implementable in realistic situations, where random decisions should be avoided.
We already focused on pure stationary schedulers, but what happens if we allow memory to pure schedulers?
With randomization, exponential-memory schedulers (in the query size) are sufficient and in general
already necessary for satisfying multiple reachability objectives (see e.g., \cite{EKVY07,RRS17}):
intuitively the memory records whether a target is reached or not, using one bit per objective.
%By restricting schedulers to be pure, some queries may require large and nontrivial memory while randomized positional schedulers are sufficient.
By restricting schedulers to be pure, such a memory is not sufficient and may require larger and nontrivial memory.
This is depicted in the following example.
\begin{example}\label{ex:nontrivial-memory}
	Consider MDP $\mdp$ of Figure~\ref{fig:kmemory} and the $2$-dimensional query $\multiobjquery = \tuple{\reachobjop_\geq\left(\eventually\{\state_3\}\right), \reachobjop_\geq\left(\eventually\{\state_4\}\right)}$.
	Let integer $k \in \nn$ and point $\point = \left(\left( \frac{1}{2} \right)^k, 1 - \left( \frac{1}{2} \right)^k \right)$. A positional randomized scheduler can easily achieve point $\point$: in $\state_2$, such a scheduler simply chooses action $\alpha$ with probability $\left( \frac{1}{2} \right)^k$ and action $\beta$ with probability $1 - \left(\frac{1}{2}\right)^k$. The case where we consider pure schedulers is much more different.
	A pure scheduler $\sched$ achieving $\point$ has to remember the number of steps performed before reaching $\state_2$.
	Indeed, if action $\alpha$ is chosen in $\state_2$ while the number of steps performed before reaching $\state_2$ is $l < k$, then $\probmeasure{\mdp}{\sched}\left(\eventually\{\state_4\}\right) \leq 1 - \left(\frac{1}{2}\right)^l < 1 - \left(\frac{1}{2}\right)^k$ and $\point$ is not achieved.
	A satisfying scheduler uses a memory of size $k$ as follows: if $\state_2$ is reached in $k$ steps or less, then the scheduler chooses $\beta$, and otherwise it chooses $\alpha$. %One can show that no other pure scheduler can achieve $\point$.
	Such pure schedulers are nontrivial in the sense that the size of their memory depends on values of the point they need to achieve, already for two objectives.
\end{example}


\begin{figure}[t]
	\vspace{-12mm}
	\begin{center}
		\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node
		distance=2.5cm,bend angle=45, scale=0.6, font=\normalsize]
		\tikzstyle{p1}=[draw,circle,text centered,minimum size=7mm,text width=4mm]
		\tikzstyle{p2}=[draw,rectangle,text centered,minimum size=7mm,text width=4mm]
		\tikzstyle{act}=[fill,circle,inner sep=1pt,minimum size=1.5pt, node distance=1cm]    \tikzstyle{empty}=[text centered, text width=15mm]
    \node[p1] (1) at (0,0) {$\state_1$};
	\node[p1] (2) at (4,0) {$\state_2$};
	\node[p1] (3) at (8,1) {$\state_3$};
	\node[p1] (4) at (8,-1) {$\state_4$};
	\node[act] (1a) at (2,0) {};
	%\node[empty] at ($(1a)-(0,0.4)$) {\scriptsize $\alpha$};
	\node[act] (2a) at (6,0.5) {};
	\node[act] (2b) at (6,-0.5) {};
	\node[act] (3a) at (9.5,1) {};
	\node[act] (4a) at (9.5,-1) {};
	\node[empty] at ($(2a)+(0,0.4)$) {\scriptsize $\alpha$};
	\node[empty] at ($(2b)-(0,0.4)$) {\scriptsize $\beta$};
	\node[]  (init) at (-1.6,0) {};
	\path[-latex']
	(init) edge (1)
	(1) edge (1a)
	(1a) edge node[above,xshift=0mm]{\scriptsize $0.5$} (2);
	(2) edge (2b)
	(2a) edge (3)
	(2b) edge (4)
	\draw [->] (1a) to[out=90,in=45] node[above,xshift=0mm]{\scriptsize $0.5$} (1);
	\draw [->] (2) -- (2a);
	\draw [->] (2) -- (2b);
	\draw [->] (2a) -- (3);
	\draw [->] (2b) -- (4);
	\draw [->] (3) to [out=45,in=100, looseness=2] (3a);
	\draw [->] (3a) to [out=-100,in=-45,looseness=2] (3);
	\draw [->] (4) to [out=45,in=100, looseness=2] (4a);
	\draw [->] (4a) to [out=-100,in=-45,looseness=2] (4);
		\end{tikzpicture}
		\caption{MDP where pure schedulers use nontrivial memory to satisfy multiple reachability objectives.}
		\label{fig:kmemory}
	\end{center}
	\vspace{-8mm}
\end{figure} 

Since we consider simple schedulers, their memory should be tractable and exponential or nontrivial memory should thus also be avoided. In that sense, it is natural to search for pure schedulers with bounded memory.
In the following, we present an approach that allows to reason about the Pareto front of a given query which only consider points achieved by pure bounded-memory schedulers.

A pure scheduler~$\sched$ in $\mdp = \mdptuple$ can be encoded by a \emph{Mealy machine}
$\schedtuple$ where~$\memorystates$ is a finite or infinite set
of memory states,~$\minit \in \memorystates$ the \emph{initial memory state},
$\schednextaction$ the \emph{next action function}
$\schednextaction\colon \states \times \memorystates \rightarrow \actions$ where
$\schednextaction(\state,\memorystate) \in \act{\state}$ for any~$\state\in \states$ and~$\memorystate \in \memorystates$,
and $\schedmemoryupdate$ the \emph{memory update function}
$\schedmemoryupdate \colon \memorystates \times \states \times \actions \rightarrow \memorystates$.  A scheduler is
\emph{$K$-memory} if~$|\memorystates| = K$.
The scheduler $\sched$ induces an MC $\mc{\mdp}{\sched}$ defined on the state space $\states \times \memorystates$ with initial state $(\sinit, \minit)$ such that, for any pair of states $(\state,\memorystate)$ and~$(\state',\memorystate')$, the probability of transition $(\state,\memorystate)$ to $(\state',\memorystate')$ when choosing action $\action$ is 
equal to $\transitions(\state,\action,\state') \cdot \iverson{\action = \schednextaction(\state,\memorystate)} \cdot \iverson{\memorystate' = \schedmemoryupdate(\memorystate,\state, \action)}$.

Let $\pschedsK{\mdp}{K}$ denote the set of pure $K$-memory schedulers, and $\pKach{\mdp}{\multiobjquery}{K}$ denote the set of points achievable by a pure $K$-memory scheduler $\sched \in \pschedsK{\mdp}{K}$ for a given multi-objective query $\multiobjquery$.
Moreover, we define the \emph{pure $K$-memory} Pareto front $\pKpareto{\mdp}{\multiobjquery}{K}$ which only considers points in $\pKach{\mdp}{\multiobjquery}{K}$ .

The pure bounded-memory problems we consider are the following.
\begin{nproblem}[framed]{Pure Bounded-memory Multi-objective Achievability Problem (\pbma)}
	Input: & MDP $\mdp$, $\numobj$-dimensional multi-objective query $\multiobjquery$, memory bound $K \in \mathbb{N}$, point $\point \in \pointdomain$.\\
	Output: & Yes if $\point \in \pKach{\mdp}{\multiobjquery}{K}$ holds.
\end{nproblem}

\begin{nproblem}[framed]{Pure Bounded-memory Pareto Approximation Problem (\pbpapprox)}
	Input: & MDP $\mdp$, $\numobj$-dimensional multi-objective query $\multiobjquery$, memory bound $K \in \nn$, precision $\precision > \rr_{>0}^\numobj$.\\
	Output: & An $\precision$-approximation of $\closure{\multiobjquery}{\pKpareto{\mdp}{\multiobjquery}{K}}$.% = \psach{\mdp}{\multiobjquery}$.
\end{nproblem}

\begin{remark}
	Let $K' \leq K$, from every $\sched' \in \pschedsK{\mdp}{K'}$, we can trivially construct a scheduler $\sched \in \pschedsK{\mdp}{K}$ with $K-K'$ unused memory states.
	Consequently, $\pKach{\mdp}{\multiobjquery}{K'} \subseteq \pKach{\mdp}{\multiobjquery}{K}$.
	Therefore, to reason about points achieved by pure schedulers with memory of maximal size $K$, it is sufficient to only consider $K$-memory schedulers.
\end{remark}

Our goal is now to establish a reduction from \pbma to \psma and from \pbpapprox \, to \pspapprox. The idea is that we incorporate in $\mdp$ a memory structure of bounded size that corresponds to the memory of a pure scheduler, and then construct a pure stationary scheduler in this refined MDP.

\begin{definition}[Nondeterministic memory structure]
	A nondeterministic memory structure of size $K > 0$ is a tuple $\ndmemory{K} = \ndmemorytuple$ with $|M| = K$, initial memory state $\minit \in M$, and nondeterministic memory update function $\ndmemoryupdate \colon \memorystates \to 2^\memorystates \setminus \emptyset$.
\end{definition}

Intuitively, according to a memory state $\memorystate \in \memorystates$, $\ndmemoryupdate(m)$ gives possible successors of $m$. Nondeterminism is interpreted as the fact that the successor of $m$ should depend on states or actions of a given MDP.

\begin{definition}[Product of an MDP and a nondeterministic memory structure]
An MDP $\mdp = \mdptuple$ and a nondeterministic memory structure $\ndmemory{K} = \ndmemorytuple$ form a new MDP $\mdpndmemory{K} = \mdpndmemorytuple$ with $\mdpndmemorystates = \states \times \memorystates$, $\mdpndmemorysinit = \left( \sinit, \minit \right)$, $\mdpndmemoryactions = \actions \times \memorystates$, and $\mdpndmemorytransitions\left( \left( \state, \memorystate \right), \left( \action, \memorystate' \right), \left( \state', \memorystate' \right)  \right) = \transitions\left( \state, \action, \state' \right) \cdot \iverson{\memorystate' \in \ndmemoryupdate\left( m \right)}$ for $\state, \state' \in \states$, $m, m' \in \memorystates$, and $\action \in \actions$.
\end{definition}

Intuitively, this product enriches $\mdp$ with a new level of nondeterminism corresponding to the choice of the next memory state in $\ndmemory{K}$.
Consequently, given a pure stationary scheduler $\sched'$ for $\mdpndmemory{K}$, we can construct a pure $K$-memory scheduler for $\mdp$ that records in its memory additional information brought with $\ndmemory{K}$ and updates its memory according to the current state of $\mdp$ and the memory state chosen by $\sched'$.

In order to set up an equivalence between schedulers for $\mdp$ and schedulers for $\mdpndmemory{K}$, we now consider \emph{complete} nondeterministic memory structures, \ie memory structures $\ndmemory{K} = \ndmemorytuple$ such that $\ndmemoryupdate(\memorystate) = \memorystates$ for all $\memorystate \in \memorystates$. Intuitively, such a structure allows to consider every possible pure schedulers with memory of size bounded by $|\memorystates|$ for the original MDP.
The following lemma holds.

\begin{lemma}
	Let $\mdp = \mdptuple$ be an MDP, $\ndmemory{K} = \ndmemorytuple$ be a complete nondeterministic memory structure, and $\mdpndmemory{K} = \mdpndmemorytuple$ be the product of $\mdp$ and $\ndmemory{K}$.
	There are equivalence relations between (i) schedulers $\sched \in \pschedsK{\mdp}{K}$ and $\sched' \in \psscheds{\mdpndmemory{K}}$, and (ii) events compliant with $\sched$ and $\sigma'$ such that equivalence (i) preserves the probability of events in equivalence relation (ii).
\end{lemma}

\begin{proof}
	Recall that $\states' = \states \times \memorystates$, $\actions' = \actions \times \memorystates$, and $\sinit' = \left ( \sinit, \minit \right )$.
	For the sake of readability, we consider pure stationary schedulers $\sched'$ as being functions $\sched' \colon \states' \to \actions'$.
	First, from a scheduler $\sched \in \pschedsK{\mdp}{K}$ encoded as $\tuple{\memorystates', \schednextaction, \schedmemoryupdate, \minit'}$, we can construct a scheduler $\sched' \in \psscheds{\mdpndmemory{K}}$ as follows.
	Since $\sched$ is $K$-memory, we link each memory state of $\sched$ to a memory state of $\ndmemory{K}$. So, consider w.l.o.g. that $\memorystates' = \memorystates$ and $\minit' = \minit$.
	For all $\left (\state, \memorystate\right ) \in \states \times \memorystates$, let $\action = \schednextaction(\state, \memorystate)$ and $m' = \schedmemoryupdate\left ( \memorystate, \state, \action \right )$, we define
	$\sched'\left (\state, \memorystate \right )= \left (\action,\memorystate' \right )$.
	Note that $\sched'$ is well defined using completeness of $\ndmemory{K}$: if $\action \in \actions(s)$, then $(\action, \memorystate') \in \actions'(\state, \memorystate)$ since $\ndmemoryupdate(\memorystate) = M$.
	
	Second, we can also construct a scheduler $\sched = \tuple{\memorystates', \schednextaction, \schedmemoryupdate, \minit'}$ from any scheduler $\sched' \in \psscheds{\mdpndmemory{K}}$ as follows. Let $\memorystates' = \memorystates$, and $\minit' = \minit$, for all $\state \in \states$ and $\memorystate \in \memorystates$ such that $\sched'(\state, \memorystate) = (\action, \memorystate')$, we define $\schednextaction(\state, \memorystate) = \action$, $\schedmemoryupdate(\memorystate, \state, \action) = \memorystate'$, and  $\schedmemoryupdate(\memorystate, \state, \action') = \memorystate$ for $\action' \neq \action$.
	
	These constructions form an equivalence between pure $K$-memory schedulers for $\mdp$ and pure stationary schedulers for $\mdpndmemory{K}$.
	Let $\sched \in \pschedsK{\mdp}{K}$ and $\sched' \in \psscheds{\mdpndmemory{K}}$ be two such equivalent schedulers, and let $\mc{\mdp}{\sched}$, $\mc{\left(\mdpndmemory{K}\right)}{\sched'}$ be the MCs induced respectively by $\sched$ and $\sched'$.
	Both MCs have the same state space defined on $\states \times \memorystates$ and initial state $(\sinit, \minit)$. Moreover, let $\mctransitions{\sched}$ be the transition function of $\mc{\mdp}{\sched}$ and $\mctransitions{\sched'}$ that of $\mc{\left(\mdpndmemory{K}\right)}{\sched'}$. We have 
	$\mctransitions{\sched}\left(\left(\state, \memorystate\right), \alpha, \left(\state', \memorystate'\right)\right) = \mctransitions{\sched'}\left(\left(\state, \memorystate\right), \left(\alpha, \memorystate' \right), \left(\state', \memorystate'\right)\right)$ for $\state, \state' \in \states$, $\action \in \actions$, and $\memorystate, \memorystate' \in \memorystates$.
%	with transitions of the form $(\state, \memorystate) \xrightarrow{\alpha} (\state', \memorystate')$ in $\mdp^\sched$ and $(\state, \memorystate) \xrightarrow{\alpha, \memorystate'} (\state', \memorystate')$ in $\mdpndmemory{K}^{\sched'}$.
	Modulo a bijection consisting in a renaming of actions, both MCs are thus identical.
	Consequently, probability of paths and events in $\mc{\mdp}{\sched}$ and $\mc{\left(\mdpndmemory{K}\right)}{\sched'}$ are equal.
\end{proof}

\begin{corollary}

	Let $\multiobjquery = \tuple{\obj_1, \dots, \obj_\numobj}$ be a multi-objective query for $\mdp$, and $\multiobjquery' = \tuple{\obj'_1, \dots, \obj'_\numobj}$ be a multi-objective query for $\mdpndmemory{K}$ such that for all $i \in \{1, \dots, \numobj\}$
	$\obj'_i = \rewobjop_\objrel\left(\rewstruct' \eventually \goalstates' \right)$ if $\obj_i$ is of the form $\rewobjop_\objrel(\rewstruct \eventually \goalstates)$,
	and $\obj'_i = \reachobjop_\objrel(\eventually \goalstates')$ if $\obj_i$ is of the form $\reachobjop_\objrel(\eventually \goalstates)$, 
%	with $\goalstates' = \goalstates \times \memorystates$ if $\goalstates \neq \emptyset$,  $\goalstates' = \emptyset$ otherwise, and $\rewstruct'((s, m), (a, m'), (s', m')) = \rewstruct(s, a, s')$ for $\state, \state' \in \states$, $\action \in \actions$, and $\memorystate, \memorystate' \in \memorystates$.
%	Then, $\pKach{\mdp}{\multiobjquery}{K} = \psach{\mdpndmemory{K}}{\multiobjquery'}$.
%
%Let $\multiobjquery$ be a multi-objective query for $\mdp$, and $\multiobjquery'$ be a multi-objective query for $\mdpndmemory{K}$ such that for all $i \in \{1, \dots, \numobj\}$,
%$\tupleaccess{\multiobjquery'}{i} = \rewobjop_\objrel\left(\rewstruct' \eventually \goalstates' \right)$ if $\tupleaccess{\multiobjquery}{i} = \rewobjop_\objrel(\rewstruct \eventually \goalstates)$,
%and $\tupleaccess{\multiobjquery'}{i} = \reachobjop_\objrel(\eventually \goalstates')$ if $\tupleaccess{\multiobjquery}{i} = \reachobjop_\objrel(\eventually \goalstates)$, 
with $\goalstates' = \goalstates \times \memorystates$ if $\goalstates \neq \emptyset$,  $\goalstates' = \emptyset$ otherwise, and $\rewstruct'((s, m), (a, m'), (s', m')) = \rewstruct(s, a, s')$ for $\state, \state' \in \states$, $\action \in \actions$, and $\memorystate, \memorystate' \in \memorystates$.
Then, $\pKach{\mdp}{\multiobjquery}{K} = \psach{\mdpndmemory{K}}{\multiobjquery'}$.
\end{corollary}

We now have all the ingredients to solve our pure bounded-memory problems: consider inputs $\mdp$, $\multiobjquery$ and $K \in \nn$, \pbma can be decided by solving the \psma problem for $\mdpndmemory{K}$ and $\multiobjquery'$ with the approach of Section~\ref{sec:milp}, and solving \pbpapprox \, can be performed by computing the solution of the \pspapprox \, problem for $\mdpndmemory{K}$ and $\multiobjquery'$ with the approach of Section~\ref{sec:pareto}.

\begin{remark}[Other memory patterns]
	Complete nondeterministic memory structures $\ndmemory{K}= \ndmemorytuple$ are in general necessary for problems \pbma and \pbpapprox.
	However, according to the instance, it could be sufficient to consider other nondeterministic memory update functions $\ndmemoryupdate$, implying less transitions in $\mdpndmemory{K}$ and considerably reducing the number of constraints of the \milp. For example, a nondeterministic memory structure for mdp of Figure~\ref{fig:kmemory} only requires $\delta(m_i) = \{m_i, m_{i+1}\}$ if $i < K$ and $\delta(m_i) = \{m_{i}\}$ otherwise, to achieve 
	$\point = \left(\left( \frac{1}{2} \right)^{K - 1}, 1 - \left( \frac{1}{2} \right)^{K - 1} \right)$ and satisfy $\multiobjquery = \tuple{\reachobjop_\geq\left(\eventually\{\state_3\}\right), \reachobjop_\geq\left(\eventually\{\state_4\}\right)}$ (cf. Example~\ref{ex:nontrivial-memory}). Note however that in general, with non-complete memory structure,
	%since we can recover a pure $K$-memory scheduler for $\mdp$ from any pure stationary scheduler for $\mdpndmemory{K}$,
	we only have $\psach{\mdp}{\multiobjquery} \subseteq \psach{\mdpndmemory{K}}{\multiobjquery'} \subseteq \pKach{\mdp}{\multiobjquery}{K}$. 
\end{remark}




